Modelling the Raft Distributed Consensus Protocol in mCRL2

The consensus problem is a fundamental problem in distributed systems. It involves a set of actors, or entities, that need to agree on some values or decisions. The Raft algorithm is a solution to the consensus problem that has gained widespread popularity as an easy-to-understand and implement alternative to Lamport's Paxos algorithm. In this paper we discuss a formalisation of the Raft algorithm and its associated correctness properties in the mCRL2 specification language.

==> eptcsdata.tex <==
\providecommand{\firstpage}{7}
\providecommand{\publicationstatus}{F. Lang, M. Volk (Eds):\\
Models for Formal Analysis of Real Systems (MARS 2024)\\
EPTCS 399, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.399.4}{10.4204/EPTCS.399.4}}

